Building Trust in the Quantum Cloud with Physical Unclonable Functions

As cloud-based quantum computing expands, securing access to quantum hardware is increasingly critical. We present an authentication protocol that leverages intrinsic quantum device properties to construct Quantum Physical Unclonable Functions (Q-PUFs). Using frequency fingerprints from fixed-frequency transmon qubits, we prototype our approach on IBM quantum devices with both real and simulated data. We employ fuzzy extractors to generate stable cryptographic keys that tolerate measurement noise and conceal raw hardware data. To support scalability, we introduce q tuples (qubit subsets) that enable challenge response generation for strong PUF behavior. We also outline extensions to neutral atom platforms and propose future directions including logical Q-PUFs. Our work lays the groundwork for secure, hardware-rooted authentication in hybrid quantum-classical systems.

==> tex-files/6-cold-atoms.tex <==

\section{Extensions to Cold Atom Technologies}

Orignal Q-PUF development focused on transmon qubit technologies. However, techniques can extend to cold atom technology.  Cold atom based sensors, clocks, and compute hardware that will all become critical elements in the future quantum compute ecosystem. Securing these end nodes is of high importance, especially if these elements are responsible for delivering mission-critical data while being located in potentially insecure environments. 

Just like with the transmon-based QCs, we look for intrinsic properties that can be used as a reliable and robust fingerprint. This fingerprint can later become a basis for a Q-PUF. Uniquely fingerprinting cold atom devices requires methods that differ from SC transmon technology because of the nature of the devices. For example, one of the benefits of the neutral atom (NA) quantum computing platform is that each qubit, which is an atom suspended by optical tweezers, is identical. Thus, unlike with the transmon-based QC, intrinsic features of the NA QC qubits cannot be used for device fingerprinting. This inspires us to examine other elements of the NA-based system's architecture to develop a fingerprint and corresponding Q-PUF.

Cold atom quantum devices suffer from systematic sources of imperfection that can serve as a basis for an intrinsic  Q-PUF fingerprint. In the rest of this section, we detail elements of cold atom systems that are viable sources of features that could be used for device fingerprinting. We also propose methods for feature characterization. We leave detailed analysis of the uniqueness, consistency, and collision resistance of these proposed cold atom fingerprints for future stages of this project. 

\subsection{Control Hardware}

NA quantum systems depend of sophisticated laser networks for atom cooling, trapping, addressing, and readout. Laser sources are required to be ultra-precise, but unfortunately these devices used for system control suffer from operational variation.~\cite{wintersperger2023neutral}. Specifically, laser intensity and phase noise has been observed. Laser intensity noise, which is variation in the optical power of the beam, can be characterized with a laser spectrum analyzer. Phase noise, which is variation of the optical phase of the beam, can be characterized by using a spectrum analyzer to determine the noise of the signal in the frequency domain.  

\subsection{Vapor Cell}

NA QCs as well as quantum sensors based on Rydberg atoms include a glass cell as a critical part of their architecture. It is within this glass cell where atoms are trapped within a vaccuum and manipulated for quantum information processing and sensing applications. While these glass cells are manufactured to be as defect-free as possible, finite precision in processing has potential to inject slight amounts of variation cell to cell. Certain noise channels associated with cold atom technology, such as measurement uncertainty with Rydberg atom RF sensor, are influenced by the dimensions and properties of the vapor cell~\cite{holloway2015atom}. In this example, the RF field interacts with the glass, and standing waves can develop as a result from internal reflection. Measuring these resulting standing waves could provide a means to identify a specific piece of cold atom quantum hardware. 

As a result of imprecision in fabrication, vapor cells have also been observed to have warping in glass windows~\cite{ma2020dc}. This warping is often more apparent as one approaches the outer edges of the cell wall. Rydberg electromagnetically induced transparency (EIT) spectroscopy has been used to characterize changes in absorption coefficients due to variation in the glass.
\black

